Evaluating Inter-Bilingual Semantic Parsing for Indian Languages

Despite significant progress in Natural Language Generation for Indian languages (IndicNLP), there is a lack of datasets around complex structured tasks such as semantic parsing. One reason for this imminent gap is the complexity of the logical form, which makes English to multilingual translation difficult. The process involves alignment of logical forms, intents and slots with translated unstructured utterance. To address this, we propose an Inter-bilingual Seq2seq Semantic parsing dataset IE-SEMPARSE for 11 distinct Indian languages. We highlight the proposed task's practicality, and evaluate existing multilingual seq2seq models across several train-test strategies. Our experiment reveals a high correlation across performance of original multilingual semantic parsing datasets (such as mTOP, multilingual TOP and multiATIS++) and our proposed IE-SEMPARSE suite.

==> intents_slots.tex <==
\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\begin{tabular}{m{5em}|m{20em}m{20em}}\toprule
\textbf{Dataset} &\textbf{Intents} &\textbf{Slots} \\\midrule
\textbf{\itop} &IN:GET\_MESSAGE', 'IN:GET\_WEATHER', 'IN:GET\_ALARM', 'IN:SEND\_MESSAGE', 'IN:GET\_INFO\_RECIPES', 'IN:SET\_UNAVAILABLE', 'IN:DELETE\_REMINDER', 'IN:GET\_STORIES\_NEWS', 'IN:CREATE\_ALARM', 'IN:GET\_REMINDER', 'IN:CREATE\_REMINDER', 'IN:GET\_RECIPES', 'IN:QUESTION\_NEWS', 'IN:GET\_EVENT', 'IN:PLAY\_MUSIC', 'IN:GET\_CALL\_TIME', 'IN:CREATE\_CALL', 'IN:END\_CALL', 'IN:CREATE\_PLAYLIST\_MUSIC', 'IN:CREATE\_TIMER', 'IN:IGNORE\_CALL', 'IN:GET\_LIFE\_EVENT', 'IN:GET\_INFO\_CONTACT', 'IN:UPDATE\_CALL', 'IN:UPDATE\_REMINDER\_DATE\_TIME', 'IN:GET\_CONTACT', 'IN:GET\_TIMER', 'IN:GET\_REMINDER\_DATE\_TIME', 'IN:DELETE\_ALARM', 'IN:PAUSE\_MUSIC', 'IN:GET\_AGE', 'IN:GET\_SUNRISE', 'IN:GET\_EMPLOYER', 'IN:GET\_EDUCATION\_TIME', 'IN:ANSWER\_CALL', 'IN:SET\_RSVP\_YES', 'IN:SNOOZE\_ALARM', 'IN:GET\_JOB', 'IN:UPDATE\_REMINDER\_TODO', 'IN:IS\_TRUE\_RECIPES', 'IN:REMOVE\_FROM\_PLAYLIST\_MUSIC', 'IN:GET\_AVAILABILITY', 'IN:GET\_CATEGORY\_EVENT', 'IN:PLAY\_MEDIA', 'IN:ADD\_TIME\_TIMER', 'IN:GET\_CALL', 'IN:SET\_AVAILABLE', 'IN:ADD\_TO\_PLAYLIST\_MUSIC', 'IN:GET\_EMPLOYMENT\_TIME', 'IN:SHARE\_EVENT', 'IN:PREFER', 'IN:START\_SHUFFLE\_MUSIC', 'IN:GET\_CALL\_CONTACT', 'IN:GET\_LOCATION', 'IN:SILENCE\_ALARM', 'IN:SWITCH\_CALL', 'IN:GET\_TRACK\_INFO\_MUSIC', 'IN:SUBTRACT\_TIME\_TIMER', 'IN:GET\_SUNSET', 'IN:DELETE\_TIMER', 'IN:UPDATE\_TIMER', 'IN:PREVIOUS\_TRACK\_MUSIC', 'IN:SET\_DEFAULT\_PROVIDER\_MUSIC', 'IN:HOLD\_CALL', 'IN:GET\_MUTUAL\_FRIENDS', 'IN:SKIP\_TRACK\_MUSIC', 'IN:UPDATE\_METHOD\_CALL', 'IN:SET\_RSVP\_INTERESTED', 'IN:QUESTION\_MUSIC', 'IN:GET\_UNDERGRAD', 'IN:PAUSE\_TIMER', 'IN:UPDATE\_ALARM', 'IN:GET\_REMINDER\_LOCATION', 'IN:GET\_ATTENDEE\_EVENT', 'IN:LIKE\_MUSIC', 'IN:RESTART\_TIMER', 'IN:RESUME\_TIMER', 'IN:MERGE\_CALL', 'IN:GET\_MESSAGE\_CONTACT', 'IN:REPLAY\_MUSIC', 'IN:LOOP\_MUSIC', 'IN:GET\_REMINDER\_AMOUNT', 'IN:GET\_DATE\_TIME\_EVENT', 'IN:STOP\_MUSIC', 'IN:GET\_DETAILS\_NEWS', 'IN:GET\_EDUCATION\_DEGREE', 'IN:SET\_DEFAULT\_PROVIDER\_CALLING', 'IN:GET\_MAJOR', 'IN:UNLOOP\_MUSIC', 'IN:GET\_CONTACT\_METHOD', 'IN:SET\_RSVP\_NO', 'IN:UPDATE\_REMINDER\_LOCATION', 'IN:RESUME\_CALL', 'IN:CANCEL\_MESSAGE', 'IN:RESUME\_MUSIC', 'IN:UPDATE\_REMINDER', 'IN:DELETE\_PLAYLIST\_MUSIC', 'IN:REWIND\_MUSIC', 'IN:REPEAT\_ALL\_MUSIC', 'IN:FAST\_FORWARD\_MUSIC', 'IN:DISLIKE\_MUSIC', 'IN:GET\_LIFE\_EVENT\_TIME', 'IN:DISPREFER', 'IN:REPEAT\_ALL\_OFF\_MUSIC', 'IN:HELP\_REMINDER', 'IN:GET\_LYRICS\_MUSIC', 'IN:STOP\_SHUFFLE\_MUSIC', 'IN:GET\_AIRQUALITY', 'IN:GET\_LANGUAGE', 'IN:FOLLOW\_MUSIC', 'IN:GET\_GENDER', 'IN:CANCEL\_CALL', 'IN:GET\_GROUP' &SL:', 'SL:AGE', 'SL:ALARM\_NAME', 'SL:AMOUNT', 'SL:ATTENDEE', 'SL:ATTENDEE\_EVENT', 'SL:ATTRIBUTE\_EVENT', 'SL:CATEGORY\_EVENT', 'SL:CONTACT', 'SL:CONTACT\_ADDED', 'SL:CONTACT\_METHOD', 'SL:CONTACT\_RELATED', 'SL:CONTACT\_REMOVED', 'SL:CONTENT\_EXACT', 'SL:DATE\_TIME', 'SL:EDUCATION\_DEGREE', 'SL:EMPLOYER', 'SL:GENDER', 'SL:GROUP', 'SL:JOB', 'SL:LIFE\_EVENT', 'SL:LOCATION', 'SL:MAJOR', 'SL:METHOD\_RECIPES', 'SL:METHOD\_RETRIEVAL\_REMINDER', 'SL:METHOD\_TIMER', 'SL:MUSIC\_ALBUM\_MODIFIER', 'SL:MUSIC\_ALBUM\_TITLE', 'SL:MUSIC\_ARTIST\_NAME', 'SL:MUSIC\_GENRE', 'SL:MUSIC\_PLAYLIST\_MODIFIER', 'SL:MUSIC\_PLAYLIST\_TITLE', 'SL:MUSIC\_PROVIDER\_NAME', 'SL:MUSIC\_RADIO\_ID', 'SL:MUSIC\_REWIND\_TIME', 'SL:MUSIC\_TRACK\_TITLE', 'SL:MUSIC\_TYPE', 'SL:NAME\_APP', 'SL:NEWS\_CATEGORY', 'SL:NEWS\_REFERENCE', 'SL:NEWS\_SOURCE', 'SL:NEWS\_TOPIC', 'SL:NEWS\_TYPE', 'SL:ORDINAL', 'SL:PERIOD', 'SL:PERSON\_REMINDED', 'SL:PHONE\_NUMBER', 'SL:RECIPES\_ATTRIBUTE', 'SL:RECIPES\_COOKING\_METHOD', 'SL:RECIPES\_CUISINE', 'SL:RECIPES\_DIET', 'SL:RECIPES\_DISH', 'SL:RECIPES\_EXCLUDED\_INGREDIENT', 'SL:RECIPES\_INCLUDED\_INGREDIENT', 'SL:RECIPES\_MEAL', 'SL:RECIPES\_QUALIFIER\_NUTRITION', 'SL:RECIPES\_RATING', 'SL:RECIPES\_SOURCE', 'SL:RECIPES\_TYPE', 'SL:RECIPES\_TYPE\_NUTRITION', 'SL:RECIPES\_UNIT\_MEASUREMENT', 'SL:RECIPES\_UNIT\_NUTRITION', 'SL:RECIPIENT', 'SL:SCHOOL', 'SL:SENDER', 'SL:SIMILARITY', 'SL:TIMER\_NAME', 'SL:TITLE\_EVENT', 'SL:TODO', 'SL:TYPE\_CONTACT', 'SL:TYPE\_CONTENT', 'SL:TYPE\_RELATION', 'SL:USER\_ATTENDEE\_EVENT', 'SL:WEATHER\_ATTRIBUTE', 'SL:WEATHER\_TEMPERATURE\_UNIT' \\
\textbf{\indictop} &IN:COMBINE', 'IN:GET\_CONTACT', 'IN:GET\_DIRECTIONS', 'IN:GET\_DISTANCE', 'IN:GET\_ESTIMATED\_ARRIVAL', 'IN:GET\_ESTIMATED\_DEPARTURE', 'IN:GET\_ESTIMATED\_DURATION', 'IN:GET\_EVENT', 'IN:GET\_EVENT\_ATTENDEE', 'IN:GET\_EVENT\_ATTENDEE\_AMOUNT', 'IN:GET\_EVENT\_ORGANIZER', 'IN:GET\_INFO\_ROAD\_CONDITION', 'IN:GET\_INFO\_ROUTE', 'IN:GET\_INFO\_TRAFFIC', 'IN:GET\_LOCATION', 'IN:GET\_LOCATION\_HOME', 'IN:GET\_LOCATION\_HOMETOWN', 'IN:GET\_LOCATION\_SCHOOL', 'IN:GET\_LOCATION\_WORK', 'IN:NEGATION', 'IN:UNINTELLIGIBLE', 'IN:UNSUPPORTED', 'IN:UNSUPPORTED\_EVENT', 'IN:UNSUPPORTED\_NAVIGATION', 'IN:UPDATE\_DIRECTIONS' &SL:AMOUNT', 'SL:ATTENDEE\_EVENT', 'SL:ATTRIBUTE\_EVENT', 'SL:CATEGORY\_EVENT', 'SL:CATEGORY\_LOCATION', 'SL:COMBINE', 'SL:CONTACT', 'SL:CONTACT\_RELATED', 'SL:DATE\_TIME', 'SL:DATE\_TIME\_ARRIVAL', 'SL:DATE\_TIME\_DEPARTURE', 'SL:DESTINATION', 'SL:GROUP', 'SL:LOCATION', 'SL:LOCATION\_CURRENT', 'SL:LOCATION\_MODIFIER', 'SL:LOCATION\_USER', 'SL:LOCATION\_WORK', 'SL:METHOD\_TRAVEL', 'SL:NAME\_EVENT', 'SL:OBSTRUCTION', 'SL:OBSTRUCTION\_AVOID', 'SL:ORDINAL', 'SL:ORGANIZER\_EVENT', 'SL:PATH', 'SL:PATH\_AVOID', 'SL:POINT\_ON\_MAP', 'SL:ROAD\_CONDITION', 'SL:ROAD\_CONDITION\_AVOID', 'SL:SEARCH\_RADIUS', 'SL:SOURCE', 'SL:TYPE\_RELATION', 'SL:UNIT\_DISTANCE', 'SL:WAYPOINT', 'SL:WAYPOINT\_ADDED', 'SL:WAYPOINT\_AVOID' \\
\textbf{\indicatis} &IN:FLIGHT', 'IN:FLIGHT\_TIME', 'IN:AIRFARE', 'IN:GROUND\_SERVICE', 'IN:AIRPORT', 'IN:AIRCRAFT', 'IN:AIRLINE', 'IN:DISTANCE', 'IN:GROUND\_FARE', 'IN:ABBREVIATION', 'IN:QUANTITY', 'IN:CITY', 'IN:FLIGHT\_NO', 'IN:CAPACITY', 'IN:FLIGHT+AIRFARE', 'IN:MEAL', 'IN:RESTRICTION', 'IN:AIRLINE+FLIGHT\_NO', 'IN:GROUND\_SERVICE+GROUND\_FARE', 'IN:AIRFARE+FLIGHT\_TIME', 'IN:CHEAPEST', 'IN:AIRCRAFT+FLIGHT+FLIGHT\_NO' & \\
\bottomrule
\end{tabular}
\end{table}

==> motivation.tex <==

\section{Further Discussions}
\label{sec:further-discussion-appendix}

\paragraph{Why \emph{Indic} languages?} Indic languages are spoken by more than a billion people in the Indian subcontinent. With the introduction of IndicNLPSuite \citep{kakwani-etal-2020-indicnlpsuite} by AI4Bharat\footnote{\url{https://ai4bharat.org}} there has been has an increased interest and effort towards the research for \emph{Indic} languages model. Recently, IndicBERT, MuRIL \citep{khanuja2021muril} based on BERT \citep{devlin2019bert} were introduced for the \emph{Indic} languages. Furthermore, generation model IndicTrans \citep{ramesh2021samanantar} and IndicBART \citep{dabre2021indicbart} based on seq2seq architecture was also published recently. These model use the \emph{Indic} enrich monolingual corpora: Common Crawl, Oscar and IndicCorp and parallel corpora: Samantar and PMIndia \citep{haddow2020pmindia} on \emph{Indic} languages for training.  Despite significant progress through large transformer-based \emph{Indic} language models in addition to existing multilingual models e.g. mBERT \citep{devlin2019bert} , XLM-RoBERTa \citep{conneau2020unsupervised}, and mBART (seq2seq) \cite{liu-etal-2020-multilingual-denoising} there is currently a paucity of benchmark data-sets for evaluating these huge language models in the \emph{Indic} language research field. Such benchmark dataset is necessary for studying the linguistic features of Indic languages and how well they are perceived by different multilingual models.  Recently, IndicGLUE \cite{kakwani-etal-2020-indicnlpsuite} was introduced to handle this scarcity. However, the scope of this benchmark, is confined to only few tasks and datasets.

% 

\paragraph{Why \datasetName task?} This research provides an excellent chance to investigate the efficacy of various Multilingual models on \emph{Indic} languages that are rarely evaluated or explored before. Some of these \emph{Indic} languages such as \emph{`Assamese'} and \emph{`Odia'} serve as unseen (zero-shot) evaluation for models such as mBERT \citep{pires-etal-2019-multilingual}, i.e. not pre-trained on \emph{`Assamese'}. While other models, such as XLM-RoBERTa, IndicBERT and MuRIL covers all our languages but in widely varying proportions in their training data. Our work investigate the correlation effect of cross-lingual training for English on these rare \emph{Indic} languages, which are not explore by prior studies. Furthermore, we also investigate the cross-lingual transfer effect across \emph{Indic} languages, also not explored before. We explore the impact of Multilingual training, english-data augmentation, unified Indic model performance, cross-lingual transfer of closely related \emph{Indic} family  and English-\emph{Indic} NLI through our work. All the above mention topics are not explore for \emph{Indic} language before. We aim to integrate \datasetName and benchmark models in IndicGLUE \cite{kakwani-etal-2020-indicnlpsuite}. Such a benchmark dataset is required for investigating the linguistic properties of Indian languages and how accurately they are interpreted by various multilingual models. Another direction is accessing model performance on {\sc Indic-IndicXNLI} task,  where both premises and hypothesis are in two distinct \emph{Indic} languages. 

% \paragraph{Why Multilingual NLI?} \da{maybe we can remove this we have already talked about this in introduction} Natural Language Inference (NLI) is a task where we are given two sentences, premise and hypothesis and the model has to predict if the premise entails or negates the sentence or does neither. NLI is a classical approach for evaluating the reasoning ability of NLP models. Recently, {\sc XNLI} \citep{conneau2018xnli} a dataset sampled from MultiNLI dataset  was created with an intent to evaluate the cross-lingual Multilingual models for several languages. However, this dataset covers only \emph{`Hindi'} in \emph{Indic} languages family. \emph{`Hindi'} although being a prominent language in the Indian subcontinent, is not the native language of many Indians and differs morphologically from languages such as \emph{`Tamil'}, \emph{`Malayali}, and \emph{`Telugu'}, which we considered for this study.

\paragraph{Why IndicTrans for Translation?}
\label{why_indicTrans_appendix}
% % \begin{itemize}
We use the IndicTrans as a translation model for converting English {\sc XNLI} to \datasetName because of the following reasons: \begin{inparaenum}[(a.)]
\item \textbf{Open-Source:} IndicTrans is open-source to public for non-commercial usage without additional fees, while Google-Translate and Microsoft-Translate require paid subscription. 
\item \textbf{Light Weight:} IndicTrans is the fastest and the lightest amongst mBART and mT5 on single-core GPU machines. Google-Translate and Microsoft-Translate are also relatively slower due to repeated network-intensive API calls.
\item \textbf{\emph{indic} Coverage:} Seq2Seq models like mBART and mT5 are not designed for all languages in the indic family. mBART supports eight (excludes kn,or,pa,as) while mT5 supports nine languages (excludes or,as) out of eleven indic languages. Google-Translate supports ten out of eleven \emph{indic} languages (excludes Assamese). Microsoft Translate supports all the eleven \emph{indic} languages.
\end{inparaenum} In future, we plan to enhance \datasetName with better translation methods.



==> tables_dataset_retention.tex <==
\begin{table*}[htbp!]
\centering
\scriptsize
\begin{tabular}{l|cc|ccccccccccc}\toprule
&\textbf{Dataset} & Original Size &\textbf{as} &\textbf{bn} &\textbf{gu} &\textbf{hi} &\textbf{kn} &\textbf{ml} &\textbf{mr} &\textbf{or} &\textbf{pa} &\textbf{ta} &\textbf{te} \\
\midrule
&\textbf{\itop} & 4386 &2574 &2253 &2109 &2123 &2217 &1975 &2123 &1772 &2300 &2058 &2177 \\
\textbf{Size}&\textbf{\indictop} & 9042& 6686 &6399 &6276 &4652 &6121 &6103 &5812 &5261 &6850 &6025 &5961 \\
&\textbf{\indicatis} &896 &793 &689 &735 &718 &658 &685 &631 &578 &750 &692 &681 \\
\hdashline
&\textbf{\itop} & 4386&59 &51 &48 &48 &51 &45 &48 &40 &52 &47 &50 \\
\textbf{Percentage}&\textbf{\indictop} & 9042&74 &71 &69 &51 &68 &67 &64 &58 &76 &67 &66 \\
&\textbf{\indicatis} &896 &89 &77 &82 &80 &74 &77 &71 &65 &84 &77 &76 \\
\bottomrule
\end{tabular}
\caption{Size and Percentage of Test Data Retained after Filteration}\label{tab: percentage retain}
\end{table*}

\begin{table*}[htbp!]
\centering
\scriptsize
\begin{tabular}{l|ccccccccccc}\toprule
\textbf{Dataset} &\textbf{as} &\textbf{bn} &\textbf{gu} &\textbf{hi} &\textbf{kn} &\textbf{ml} &\textbf{mr} &\textbf{or} &\textbf{pa} &\textbf{ta} &\textbf{te} \\
\midrule
\textbf{\itop} &1287 &1127 &1055 &1062 &1109 &988 &1062 &886 &1150 &1029 &1089 \\
\textbf{\indictop} &3343 &3200 &3138 &2326 &3061 &3052 &2906 &2631 &3425 &3013 &2981 \\
\textbf{\indicatis} &397 &345 &368 &359 &329 &343 &316 &289 &375 &346 &341 \\
\bottomrule
\end{tabular}
\caption{Size of Dev Data Retained after Filteration}\label{tab: dev percentage retain}
\end{table*}
